Bayesian nonparametric mixture inconsistency for the number of components: How worried should we be in practice?

We consider the Bayesian mixture of finite mixtures (MFMs) and Dirichlet process mixture (DPM) models for clustering. Recent asymptotic theory has established that DPMs overestimate the number of clusters for large samples and that estimators from both classes of models are inconsistent for the number of clusters under misspecification, but the implications for finite sample analyses are unclear. The final reported estimate after fitting these models is often a single representative clustering obtained using an MCMC summarisation technique, but it is unknown how well such a summary estimates the number of clusters. Here we investigate these practical considerations through simulations and an application to gene expression data, and find that (i) DPMs overestimate the number of clusters even in finite samples, but only to a limited degree that may be correctable using appropriate summaries, and (ii) misspecification can lead to considerable overestimation of the number of clusters in both DPMs and MFMs, but results are nevertheless often still interpretable. We provide recommendations on MCMC summarisation and suggest that although the more appealing asymptotic properties of MFMs provide strong motivation to prefer them, results obtained using MFMs and DPMs are often very similar in practice.

==> Sampling.tex <==

\section{Overview}

In order to perform inference on parameters of a Bayesian mixture model we consider a Markov chain Monte Carlo (MCMC) approach.
In general, MCMC estimation consists in generating a Markov chain $\bm \phi^{(1)}, \ldots, \bm \phi^{(M)}$ of the parameters of a model.
For the mixture of finite mixtures model we have $\bm \phi = (\bm z, K, \bm \pi, \bm \theta )$ and for the Dirichlet process mixture model we have either $\bm \phi = \bm \theta$ or $\bm \phi = (\bm \theta, \alpha)$, depending on whether $\alpha$ has a prior distribution.
We generate a Markov chain such that it has the posterior as a stationary distribution, i.e.,
\begin{equation}
    \bm \phi^{(m)} \sim p\left( \bm \phi \mid X_1, \ldots ,  X_N \right), \quad m = 1, \ldots, M.
\end{equation}
 MCMC sampling is necessary for mixture models because the posterior is generally neither known nor analytically tractable. A common method for MCMC sampling, in particular for Bayesian mixture models, is Gibbs sampling. Instead of formulating a proposal of all parameters in $\bm \phi$ at every iteration, a Gibbs algorithm samples parameters of $\bm \phi$ conditionally.
Formally, we consider each parameter $\phi_\nu$ of $\bm \phi$ separately and write $\bm \phi_{-\nu}$ for the remaining parameters.
Then Gibbs sampling consists in sampling from the conditional posterior $p(\phi_{\nu} \mid \bm \phi_{-\nu}, \bm X)$ for every $\nu$ in some alternating, possibly random, order.

For the Dirichlet process mixture model, the most straightforward sampling methods use Gibbs sampling \citep{maceachern94,escobar95} and take advantage of the Dirichlet process prior. From the Polya urn scheme representation (\ref{def:polya}) the prior distribution of $\theta_i \mid \bm \theta_{-i}$ is a simple mixture, which allows us to write the unnormalised conditional posterior as
\begin{equation}
\label{eq:gibbs_sampler}
    p(  \theta_i \mid \bm \theta_{-i}, \bm X )  \propto
    \begin{cases}
    p( \bm X \mid \bm \theta), \quad \theta_i = \theta_j, j \neq i, \\
    \alpha p( \bm X \mid \bm \theta) H(\theta_i), \quad \text{otherwise},
    \end{cases}
    % \theta_i \mid \bm \theta_{-i}, \bm X \propto 
    % \frac{\alpha}{\alpha + i - 1} H(\theta_i) F \big(\bm X \mid \bm \theta \big) \delta(\theta_i \neq \theta_j, j \neq i)
    % + \frac{1}{\alpha + i - 1} \sum_{j\neq i} F \big(\bm X \mid \bm \theta \big)\delta(\theta_i = \theta_j),
\end{equation}
where the first case may be regrouped into components of identical $\theta_j$. Moreover, under conjugacy of $H$ the conditional posterior becomes tractable. In that case we can obtain Gibbs samples directly instead of relying on a Metropolis--Hastings step. Despite its simplicity the Gibbs sampling approach for the Dirichlet process mixture model is slow in practice and tends to get stuck in local modes. Indeed, its incremental updates mean that the Gibbs sampler is unlikely to explore different modes if it must first cross some low-density region. Therefore \cite{jain04} suggest a sampler which takes the whole allocation structure into account, which we present in Section~\ref{sec:sm}.

For the mixture of finite mixtures model another difficulty for sampling methods is the changing number of components.
Whenever $K$ changes all other parameters change their dimensionality accordingly. In fact, we can interpret inference of the mixture on finite mixtures model as a model selection problem.
For this reason we cannot perform straightforward Gibbs sampling as for the Dirichlet process mixture model, and updating the number of components requires a more complex update of the entire component structure.
This explains the lower popularity of the mixture of finite mixtures model relative to the Dirichlet process mixture model.
Some approaches to inferring the mixture of finite mixtures model include approximating the marginal likelihood of $K$ \citep{nobile94}, detailed Gibbs proposals \citep{nobile07}, or continuous-time birth-death processes \citep{stephens00}, which consider creation and deletion of components as birth and death events respectively.
The most popular approach remains reversible jump processes, introduced by \cite{green95} and then applied to mixture models by \cite{richardson97}.
Reversible jumps are a general solution to Metropolis--Hastings proposals for models with varying dimensionality.
While usual Metropolis-Hasting approaches force Markov chain reversibility by adjusting the acceptance probabilities, reversible jumps directly ensure detailed balance and give a construction of suitable MCMC steps when $K$ changes.
In practice reversible jumps require case-by-case derivation to assure reversibility depending on the model specification. To avoid the difficult manual search for ``good`` reversible proposals, \cite{miller18} suggest an approach based on the popular split-merge sampler for Dirichlet process mixture models. We give a summary of their method in Section~\ref{sec:mh18}.
Another efficient alternative to reversible jump MCMC is the allocation sampler \citep{nobile07}, which bears some resemblance to split-merge proposals.

% [ Eventually, mention code availability in R, Python, Julia (OFAI, DPMMSub), PPLs?]
 
 % There are a few challenges for sampling from the posterior of a mixture models. Firstly, the allocation parameters $z$ are discrete and we cannot directly use popular approaches such as Hamiltonian Monte Carlo \citep{duane87} which rely on the regularity of the posterior. Instead, for efficient 
 
\section{Split-merge sampler}
\label{sec:sm}

The split-merge sampler \citep{jain04,jain07} is an inference method for Dirichlet process mixture models, but in Section~\ref{sec:mh18} we give an adaptation for the mixtures of finite mixtures model \citep{miller18}.
We keep our notation general and denote the parameters by $\bm \phi = (\bm z, \bm \theta)$, where $\bm z$ is the component allocation and $\bm \theta = (\theta_1, \ldots, \theta_{T})$ are the $T$ distinct component parameters. With this notation we abuse the previous observation-wise indexing $\theta_i$ and write $\theta_{z_i}$ instead.
%The components $1, \ldots, T$ are usually called \emph{active} components and for simplicity
We assume that the labels are contiguous, i.e., $z_i \in \{1, \ldots, T \}$ for all $i=1, \ldots, N$, and that the prior on $\bm \theta$ satisfies conditional conjugacy, i.e., $\theta_\nu \mid \bm \theta_{-\nu}, \bm X$ follows a known distribution, so we can directly obtain a conditional Gibbs sample.

We describe how to obtain samples $\bm \phi^{(1)}, \ldots, \bm \phi^{(M)}$ with the split-merge sampler as an increment from $\bm \phi^{(m)}$ to $\bm \phi^{(m+1)}$ according to the following steps.

\vspace{4mm}
\noindent\hrulefill

\vspace{1mm}
\noindent\textbf{Split-merge algorithm}

\noindent\hrulefill
\vspace{2mm}

\noindent \textbf{1. Initiation}

Let $\bm \phi = (\bm z, \bm \theta)$ be the current sample with $T$ components.
Choose two observations $i$ and $j$ at random and assume without loss of generality that $z_i \leq z_j$, and define
$$
S = \{ l = 1, \ldots, N : z_l = z_i \text{ or } z_l = z_j \}, \quad \tilde S= S \setminus \{ i,j \}.
$$
For all further steps we only work with $S$ and aim to split or merge the observations $S$ depending on whether $z_i = z_j$ or $z_i \neq z_j$ respectively. To do so, we first construct intermediate \emph{launch} states $\bm \phi^{\text{L-split}}$ and $\bm \phi^{\text{L-merge}}$ in Steps 3 and 4 to then obtain Metropolis--Hastings proposals $\bm \phi^{\text{split}}$ and $\bm \phi^{\text{merge}}$. Despite their name, it is necessary to sample both launch states for Step 8 regardless of whether we proceed with a split or merge proposal.\vspace{2mm}

\noindent\textbf{2. Construction of} $\bm \phi^{\text{L-merge}} = \big(\bm z^{\text{L-merge}}, \bm \theta^{\text{L-merge}}\big)$

Set $z_l^{\text{L-merge}} = z_i$ for all $l \in S$ to obtain a single merged component of all observations in $S$ and sample its parameter $\theta_{z_i}^{\text{L-merge}}$ from the prior $H$. If $z_i = z_j$ then all observations in $S$ are already in a single component and the merge step keeps $\bm z$ unchanged, i.e., $\bm z^{\text{L-merge}} = \bm z$. Then, update $\bm \phi^{\text{L-merge}}$ by taking $n_{\text{merge}}$ parameter update steps as described in Step 5, which leaves $\bm z^{\text{L-merge}}$ unchanged. By default we choose $n_{\text{merge}} = 5$.\vspace{2mm}

\noindent\textbf{3. Construction of} $\bm \phi^{\text{L-split}} = \big(\bm z^{\text{L-split}}, \bm \theta^{\text{L-split}}\big)$

If $z_i \neq z_j$ then set $z_i^{\text{L-split}} = z_i$ and $z_j^{\text{L-split}} = z_j$ as the two components for the split of $S$. Otherwise, if $z_i = z_j$, set $z_i^{\text{L-split}} = z_i$ and let $z_j^{\text{L-split}} = T+1$ so that we create a new component.
For every $l \in \tilde S$ choose $z_l^{\text{L-split}}$ at random between $z_i^{\text{L-split}}$ and $z_j^{\text{L-split}}$ in order to split $S$ into two components containing $i$ and $j$ respectively.
Then, sample initial $\theta_{z_i}^{\text{L-split}}$ and $\theta_{z_j}^{\text{L-split}}$ from the component prior $H$. Update $\bm \phi^{\text{L-split}}$ by taking $n_{\text{split}}$ update steps, each consisting in a restricted Gibbs step on $\bm z^{\text{L-split}}$ described in Step 4 followed by a component parameter update described in Step 5. By default we choose $n_{\text{split}} = 5$.\vspace{2mm}

\noindent\textbf{4. Restricted Gibbs sampling}

To perform a restricted Gibbs update we sample from the conditional allocation distribution, but restrict ourselves to observations in $S$. This restriction makes the conditional distribution tractable as we only consider the two possible components $z_i^{\text{L-split}}$ and $z_j^{\text{L-split}}$. Under this restriction,
\begin{equation}
\label{eq:rgibbs}
   p(z_l = z_i \mid z_{-k}, \bm X ) = \frac{n_{-l,i} \,p(\bm X \mid \theta,\bm z_{-l},z_l = z_i )}{n_{-l,i} \,p(\bm X \mid \theta,\bm z_{-l},z_l = z_i ) + n_{-l,j} \,p(\bm X \mid \theta, \bm z_{-l},z_l = z_j)}, \quad l \in \tilde S,
\end{equation}
where $n_{-l,i} = \lvert\{ g \in S : g \neq l, z_g = z_i \}\rvert$ is the number of observations in component $z_i$ excluding $l$. Hence we sample a new allocation $z_l$ for every $l \in \tilde S$, which in total amounts to a single restricted Gibbs step.\vspace{2mm}

\noindent\textbf{5. Update component parameters}

To update the component parameters $\theta_{z_i}$ and $\theta_{z_j}$ --- or only $\theta_{z_i}$ for a merge launch state --- we use conditional conjugacy.
Assuming, for example, that $\theta = (\gamma , \eta )$, we perform Gibbs updates for $\gamma$ and $\eta$ separately, since $\gamma \mid \eta, \bm X, \bm z$ and $\eta \mid \gamma, \bm X, \bm z$ both have known distributions as a consequence of conditional conjugacy. In general, we sample from each parameter in $\theta_{z_i}$ and $\theta_{z_j}$ sequentially, which finally amounts to a single parameter update step.\vspace{2mm}

\noindent\textbf{6. Merge proposal ($z_i \neq  z_j$)}

If $z_i \neq z_j$, sample a merge proposal $\bm \phi^{\text{merge}}$ from the merge launch state $\bm \phi^{\text{L-merge}}$.
For all observations $l \in S$ propose a single component $z_l^{\text{merge}} = z_l^{\text{L-merge}} = z_i$. Keep all other parameters unchanged, i.e., for $l \in \{1, \ldots , N \} \setminus S$ keep $z_l^{\text{merge}} = z_l$ and for $k \neq z_i$, $\theta_k^{\text{merge}} = \theta_k$.
From the launch component parameter $\theta_{z_i}^{\text{L-merge}}$ perform a single additional parameter update according to Step 5 to obtain a proposal $\theta_{z_i}^{\text{merge}}$.\vspace{2mm}

\noindent\textbf{7. Split proposal ($z_i = z_j$)}

If $z_i = z_j$, sample a split proposal $\bm \phi^{\text{split}}$ from the split launch state $\bm \phi^{\text{L-split}}$ by performing a single additional update as in Steps 4 and 5. Then, for observations $l \in S$ we have $z_l^{\text{split}} \in \{ z_i, z_j \} = \{ z_i, T + 1 \}$ and for all other $l \in \{1, \ldots , N \} \setminus S,z_l^{\text{split}} = z_l$ is unchanged.
\vspace{2mm}

\noindent\textbf{8. Acceptance probabilities }$a(\bm \phi^{\text{merge}}, \bm \phi)$ \textbf{and} $a(\bm \phi^{\text{split}}, \bm \phi)$

The Metropolis--Hastings acceptance probability for a proposal $\bm \phi^* = \bm \phi^{\text{merge}}$ or $\bm \phi^* = \bm \phi^{\text{split}}$ is
\begin{equation}
    a(\bm \phi^*, \bm \phi) = \min \left[ 1, \frac{q( \bm \phi \mid \bm \phi^*)}{q ( \bm \phi^* \mid \bm \phi)} \frac{p(\bm \phi^* \mid \bm X)}{p(\bm \phi \mid \bm X )}\right],
\end{equation}
where $q$ is the transition probability and $p(\bm \phi \mid \bm X )$ is the posterior density. As usual, for the latter we only have access to the unnormalised posterior $p(\bm \phi \mid \bm X ) = p(\bm z ) p (\bm \theta ) p( \bm X \mid \bm \theta, \bm z )$, where $p( \bm z )$ is the allocation prior given in (\ref{def:polya}) and $p(\bm \theta)$ is the product of the component priors $H$ for each component $\theta_k$. The likelihood $p( \bm X \mid \bm \theta, \bm z )$ is determined by the component distribution $F$.
Since all parameters linked to observations in $\{1, \ldots, N\} \setminus S$ are constant through split-merge proposals, they cancel in the posterior ratio, and the computation of $ a(\bm \phi^*, \bm \phi)$ depends only on observations in $S$ and the two components involved in the split-merge procedure.

The proposal probability $q( \bm \phi^* \mid \bm \phi)$ only considers the transition from the launch state $\bm \phi^{\text{L-}*}$ to the proposal $\bm \phi^*$. The construction of the launch state is only an intermediate step from which we get the proposal during the final additional Gibbs sample.
In other words, the construction of the launch state could be deterministic or come from a sampling algorithm other than Gibbs sampling, though this might lead to a lower acceptance probability, and can be considered similarly to the random choice of $i$ and $j$ during Step 1. For the merge proposal, when $z_i \neq z_j$, we have
\begin{equation}
    q \left( \bm \phi^\text{merge} \mid \bm \phi \right) = p\left( \bm \theta^\text{merge} \mid \bm \theta^\text{L-merge},\bm z^\text{L-merge}, \bm X\right),
\end{equation}
which is the product of the conditional Gibbs updates for each parameter of $\bm \theta$ in Step 5.
The transition probability does not depend on $z$, as it stays constant for the merge proposal. For the split proposal,
\begin{equation}
    q\left( \bm \phi^\text{split} \mid \bm \phi\right) = p\left( \bm \theta^\text{split} \mid \bm \theta^\text{L-split},\bm z^\text{L-split}, \bm X\right) p\left( \bm z^\text{split} \mid \bm \theta^\text{L-split},\bm z^\text{L-split}, \bm X\right),
\end{equation}
where the second transition probability on $\bm z$ is a product of probabilities \eqref{eq:rgibbs} in Step 4 over the observations $\tilde S$.

To compute the reverse transition probability $q( \bm \phi \mid \bm \phi^*)$ we need to compute the probability of obtaining our initial parameters $\bm \phi$ from the proposal under the split-merge procedure. The construction of a merge launch state for a merge proposal gives the appropriate probability of reversing the launch state construction and vice-versa for the split proposal.
Suppose first that initially $z_i = z_j$, which leads to a split proposal. In this case the reversal of a split configuration always leads to a single merged component. Therefore, to compute $q( \bm \phi \mid \bm \phi^\text{merge})$ we only need to reverse the parameter updates from Step 5. Formally
\begin{equation}
\label{eq:rev_split}
    q\left( \bm \phi \mid \bm \phi^\text{split}\right) = p\left( \bm \theta \mid \bm \theta^\text{L-merge}, \bm z^\text{L-merge}, \bm X \right),
\end{equation}
where the transition probability only considers $\theta_{z_i}$, as a product of the conditional Gibbs densities in Step 5.
On the other hand, for the the merge proposal when $z_i \neq z_j$, we also take into account the restricted Gibbs updates of $\bm z$. Hence, we have
\begin{equation}
\label{eq:rev_merge}
    q\left( \bm \phi \mid \bm \phi^\text{merge}\right) =  p\left( \bm \theta \mid \bm \theta^\text{L-split}, \bm z^\text{L-split}, \bm X \right)
     p\left( \bm z \mid \bm z^\text{L-split}, \bm \theta^\text{L-split}, \bm X \right),
\end{equation}
where the transition probability for $\bm \theta$ is a product of the conditional probabilities in Step 5 over the parameters of $\theta_{z_i}$ and $\theta_{z_j}$, and the transition probability for $\bm z$ is a product of the restricted Gibbs probabilities \eqref{eq:rgibbs} over $\tilde S$.\vspace{2mm}

% when , we also construct a split launch state $\bm \phi^{\text{L-split}}$ track of the transition probabilities from the $n_* = n_\text{merge}, n_\text{split}$ Gibbs updates in Steps 4 and 5. We write $\bm \phi^{\text{L-}*,0} = (\bm z^{\text{L-}*,0}, \bm \theta^{\text{L-}*,0})$ for the initial launch states in Steps 2. and 3 and $\bm \phi^{\text{L-}*,q}$ for the $q$-th update step for $q = 1, \ldots, n_*$. Then

\noindent\textbf{9. Update hyperparameters (optional)}

If we use hyperpriors on the parameters $\bm \theta$ or on $\alpha$ we perform Gibbs sampling steps between split-merge iterations.
For $\alpha$ the conditional posterior is
\begin{equation}
    p(\alpha \mid T ) \propto \alpha^T \frac{\Gamma (\alpha) }{ \Gamma (\alpha + N )} p(\alpha), \quad \alpha > 0,
\end{equation}
where $p(\alpha)$ is a prior on $\alpha$ and $\Gamma$ is the gamma function.

\noindent\hrulefill

While conditional conjugacy is not necessary to sample proposals in the split-merge algorithm, it becomes relevant in Step 8 where we need to compute the acceptance probability. Without conditional conjugacy we cannot compute the reverse transition probabilities in (\ref{eq:rev_split}) and (\ref{eq:rev_merge}). In fact, this is one reason for the efficiency of the split-merge sampler. By updating the parameters before sampling a proposal we move into a higher density region of the posterior and thereby increase the acceptance probability. To keep the transition probabilities tractable, we also rely on the restricted Gibbs sampling in Step 4. If instead we consider all possible allocations, we require the intractable probability of creating a new component in (\ref{eq:gibbs_sampler}), which has no closed form except under full conjugacy. As a solution to this for non-conjugate cases, restricted Gibbs sampling only considers two existing components, which leads to straightforward likelihood ratios in (\ref{eq:rgibbs}).

Under full conjugacy of the component prior $H$ with the component distribution $F$ the split-merge sampler can be simplified. This corresponds to the first version of the algorithm by \cite{jain04}. In this case we can skip the conditional Gibbs sampling in Step 5 and sample $\bm \theta$ directly from the posterior conditional on $\bm z$.

There are various extensions of the split-merge sampler. For example, \cite{dahl21s} suggest constructing the split launch state with sequential allocation of observations in $S$ instead of a random split. This leads to increased computational cost, but proposals tend to be accepted more often, giving a more efficient sampler overall.

% [in the full conjugacy case we do not need to update parameters as in step 4: acceptance probabilities are known]

\section{Sampling mixture of finite mixtures models}
\label{sec:mh18}

\cite{miller18} translate any sampling method for the Dirichlet process mixture model to a sampling method for the mixture of finite mixtures model by studying a common representation for partition models. We can thereby use the popular sampling efficiency of Dirichlet process mixture samplers, such as the split-merge sampler in Section~\ref{sec:sm}. To summarise their results we give a translation of the Pólya urn scheme \eqref{def:polya} for a mixture of finite mixtures.
\begin{theorem}
\citep{miller18}\\
Let $z_1, \ldots, z_N$ be allocation parameters of a mixture of finite mixtures model. Then, for every $i = 1, \ldots, N$ and writing $t = \max_{j < i} z_j$, the conditional prior on $\bm z$ is
\begin{equation}
\label{eq:mfm_urn}
    p (z_i = k \mid z_1, \ldots, z_{i-1}) \propto 
    \begin{cases}
        \big\lvert \{ j<i \, : \, z_j = k \} \big\rvert + \gamma, \quad k \in \{z_1, \ldots, z_{i-1}\}, \\[6pt]
        \mathlarger{\frac{V_i(t+1)}{V_i(t)} \gamma}, \quad \text{otherwise,}
    \end{cases}
\end{equation}
where
\begin{equation}
    V_i(t) = \sum_{k=t}^\infty \frac{\Gamma (k+1)}{\Gamma(k-t+1)} \frac{\Gamma(k \gamma)}{\Gamma ( k \gamma + N)}.
\end{equation}
\end{theorem}
From this representation, a mixture of finite mixtures model is very similar to the Dirichlet process mixture model.
Since all considerations for the split-merge sampler also apply to the mixture of finite mixtures model, it suffices to replace the allocation prior $p( \bm z)$ in Step 8 of the algorithm with the probabilities in (\ref{eq:mfm_urn}).
Likewise, we adjust the restricted Gibbs update in Step 4 by replacing the terms $n_{-l,i}$ by $n_{-l,i} + \gamma$.  The infinite sum to obtain $V_i(t+1)$ decays rapidly and can therefore be approximated using an appropriate truncation.

To then obtain a posterior on $K$, \cite{miller18} show that, given the number of active components $T$,
\begin{equation}
\label{eq:k_post}
    p( K = k \mid T = t) = \frac{1}{V_N(t)} \frac{\Gamma (k+1)}{\Gamma(k-t+1)} p_K(k), \quad k \geq t,
\end{equation}
Moreover, conditionally on $T$, $K$ is independent of the observations $\bm X$ and allocations $\bm z$.
The difference between $T$ and $K$ is subtle: while $T$ defines the number of non-empty components, $K$ may be larger when there are empty components. However, \cite{miller18} show that, conditionally on $X_1, \ldots, X_N$, $K$ and $T$ have the same distribution as $N \rightarrow \infty$, i.e., there are almost surely no empty components under the posterior as $N \rightarrow \infty$. 

% \section{Summary methods}

% [overview of summary methods available]\\[0pt]
% [mcclust]\\[0pt]
% [mcclust.ext]\\[0pt]
% [salso]\\[0pt]
% [Premium]\\[0pt]
% [GreedyEPL]


